Reinforcement learning based demand charge minimization using energy storage

Utilities have introduced demand charges to encourage customers to reduce their demand peaks, since a high peak may cause very high costs for both the utility and the consumer. We herein study the bill minimization problem for customers equipped with an energy storage device and a self-owned renewable energy production. A model-free reinforcement learning algorithm is carefully designed to reduce both the energy charge and the demand charge of the consumer. The proposed algorithm does not need forecasting models for the energy demand and the renewable energy production. The resulting controller can be used online, and progressively improved with newly gathered data. The algorithm is validated on real data from an office building of IFPEN Solaize site. Numerical results show that our algorithm can reduce electricity bills with both daily and monthly demand charges.

==> content/application.tex <==
\label{section 4}


Our objective is to minimize electricity bills composed of fixed subscription fees, energy charges and demand charges. Energy charges represent the cost of the total amount of energy exchanged with the grid. Demand charges are based on the maximum electricity demand during a billing period, which may be one day or one month. Such a bill has the following form:


\begin{equation}
    \label{eqn: bill}
    \begin{aligned}
    \text{fees} &+ \underbrace{\mu \; \underset{t\in BP}{\text{max}} \left\{P^+_\text{meter}(t) \right\}}_\text{demand charges} \\
    &+ \underbrace{\int_{t\in BP} pp(t)P^+_\text{meter}(t) - sp(t)P^-_\text{meter}(t) \, dt}_\text{energy charges}
\end{aligned}
\end{equation}
where fees represent fixed subscription fees, $P_{meter} [kW] $ is the power exchanged with the grid, $P_{meter}^+=\text{max}(0, P_{meter})$ and $P_{meter}^-=-\text{min}(0, P_{meter})$ are the positive and the negative parts of $P_{meter}$, $pp[\$ / kWh]$ and $sp [\$ / kWh]$ are the purchase and selling prices of energy, and $\mu [\$/kW]$ is a price per kilowatt. 
In the rest of the paper, we assume that the electricity prices $pp(\cdot)$ and $sp(\cdot)$ follow a daily pattern: their values depend on the hour and remain the same for each day.

We consider a consumer equipped with a solar panel and a battery whose interactions with the grid are illustrated in Fig. \ref{fig: system}. The electricity meter centralizes the power flows. It supplies the consumption $P_{cons} [kW]$ to the user and   
 the charging power $P_{c,bat} [kW]$ to the battery and receives the solar power production $P_{pv} [kW]$ from the solar panel, the discharging power $\rho_d P_{P_{d,bat}} [kW]$ from the battery and $P_{meter}$ from the grid. $\rho_d [-]$ is the discharge efficiency of the battery: the electricity meter only receives a fraction $\rho_d$ of what the battery provides. Thus, the total balance power is given by
\begin{equation}
    \label{eq: Pmeter}
    P_{meter} = P_{cons} - P_{pv} + P_{c, bat} - \rho_d P_{d, bat}
\end{equation}
When $P_{meter}$ is positive, that amount of power is bought from the grid. When negative, it is sold. 


\begin{figure}[H]
	\centering
  	\includegraphics[scale=0.4]{img/annotated_system.png}
   \caption{Sketch of the system}
    \label{fig: system}
\end{figure}


% \subsection{Nomenclature}
% \begin{itemize}
% 	\item $x\in [0, 1]$ $[-]$: state of charge of the battery 
% 	\item $P_{c,bat}$ (resp. $P_{d,bat}$) $[kW]$: battery charge (resp. discharge) power
%     \item $pp$ (resp. $sp$) $[\$/kWh]$: energy purchase (resp. selling) price
%     \item $\mu_d$ (resp $\mu_m$) $[\$/kW]$: demand charge rate for daily (resp monthly) assessments
%     \item $\rho_d$ $[-]$: discharge efficiency of the battery
%     \item $P_{pv}$ (resp $P_{cons}$) $[kW]$: electricity production (resp. consumption)
%     \item $f^+$ and $f^-$: positive and negative part of a function or number $f$ respectively
% \end{itemize}


\subsection{Optimization criteria}
We will study  three bill minimization problems: daily energy minimization, daily  demand charge minimization, and monthly  demand charge minimization. The first one has been studied as an intermediate step towards demand charge minimization problems. Since subscription fees are fixed, they are excluded from the analysis. More precisely, the minimization criteria of these three problems are given as follows:

\subsubsection{Daily energy charges minimization}
no demand charges are involved here. The problem is to minimize the energy charge $C^{day}_{cons}$ given by:
\begin{equation}
    \label{eqn: demand charge min}
    \int_{t\in day} \left[pp(t) P_{meter}^+(t)- sp(t)P_{meter}^-(t)\right] \text{dt}
\end{equation}
 Recall that $P_{meter}^+$ and $P^-_{meter}$ are the bought and sold power respectively, and $pp$ and $sp$ are the purchase and selling energy prices.

To minimizing \eqref{eqn: demand charge min} by RL algorithms, a natural choice of the immediate cost function is the energy charge of one time step, i.e.,
\begin{equation}
        \begin{aligned}
            \label{eq: cost function crit 1}
            \mathcal{C}^1_\tau(x, a)&= \int_{t=\tau\Delta t}^{(\tau+1)\Delta t} pp(\tau)P^+_{meter}(t, a) \, dt \\ & -\int_{t=\tau\Delta t}^{(\tau+1)\Delta t} sp(\tau)P^-_{meter}(t, a) \, dt
        \end{aligned}
    \end{equation}
    % for choosing action $a$ at time step $\tau\in\mathcal{T}$ while in state of charge $x$.
    % $P_{meter}$ is defined by \eqref{eq: Pmeter}. 
  

\subsubsection{Daily demand charges minimization} the problem is to minimize $C^{day}_{dem+cons}$ which is defined as the sum of the energy charge $C^{day}_{cons}$ and the daily demand charge, i.e.
    \begin{equation}
        \label{eqref: daily demand and consumption charges}
        C^{day}_{cons} + \underset{t\in \text{day}}{\text{max}} \left\{ P^+_{meter}(t) \right\} \cdot \mu_{d}
    \end{equation}
where $\mu_d [\$/kW]$ is the demand charge rate for daily demand charges.

The immediate cost for RL is defined as:
\begin{equation}
    \label{eq: cost function crit 2}
    \mathcal{C}^2_\tau(p, x, a)=\mathcal{C}^1_\tau(x, a) + (p'-p)^+\mu_d
\end{equation} 
% with $\mu_d$ the demand charge price and 
with $p'$ the new maximal measured peak after the transition. 
This corresponds to \eqref{eqref: daily demand and consumption charges} applied to one time step.
% the demand charges computed that way to avoid having to track the whole history of peaks. 
Since the real demand peak can be observed only at the end of the billing period, we define the immediate cost of the demand charge by the increment of the peak $(p^{'}-p)^+$: an action leading to a higher peak has a larger cost. Thus, at the end of the day, the demand charge does correspond to the highest peak.
    
\subsubsection{Monthly demand charges minimization} the problem is to minimize $C^{month}_{dem+cons}$ which is defined as the sum of the energy charge of the whole month and the monthly demand charge, i.e.,
    \begin{equation}
        \label{eqref: monthly demand and consumption charges}
        \sum_{day \in BP} C^{day}_{cons} + \underset{t\in day, day \in BP}{\text{max}} \left\{ P^+_{meter}(t) \right\} \cdot \mu_{m}
    \end{equation}
where $\mu_m [\$/kW]$ is the monthly demand charge rate and $BP$ is a billing period of a month. 

The immediate cost for RL is designed as follows:

\begin{equation}
    \label{eq: cost function crit 3}
    \mathcal{C}^3_\tau(p, x, a)=\mathcal{C}^1_\tau(x, a) + (p'-p)^+\mu_m
\end{equation} 
% with $\mu_m$ the associated demand charge price. 
This cost function comes from \eqref{eqref: monthly demand and consumption charges} applied to one time step.
% and the demand charge is computed as previously. 


Note that the second term representing the demand charges in \eqref{eq: cost function crit 2} and \eqref{eq: cost function crit 3} are the same. However, the way to reset the recorded peak $p$ is different:  for daily demand charge case, $p$ is reset to zero at the beginning of each day; for monthly demand charge case, $p$ is reset to zero only at the beginning of the month.
 
\subsection{Simulation model}
% We consider a battery with a non-linear dynamic 
In order to minimise the electricity bill under realistic conditions, we consider a non-linear dynamic model of the battery
\cite{Dynamic_Battery}. At time $t \in \mathbb{R}^+$, the state of charge (SOC) of the battery $x [-]$ changes according to the following equation:
\begin{equation}
\label{eqn:x_dot}
\dot{x}(t)=\frac{I_{bat}(t)}{Q_{bat}^{nominal}} \left[s^{-1}\right]
\end{equation}
with $Q_{bat}^{nominal}[As]$ the nominal charge capacity of the battery and $I_{bat} [A]$ the current of the battery given by
\begin{equation}
\label{eqn:Ibat}
\begin{cases}
\frac{-U_{ocv}(x)+\sqrt{U_{ocv}(x)^2+4R_{c,int}(x)P_{c,bat}(t)}}{2R_{c,int}(x)} & \text{(charge)}\\
\frac{-U_{ocv}(x)+\sqrt{U_{ocv}(x)^2-4R_{d,int}(x)P_{d,bat}(t)}}{2R_{d,int}(x)} & \text{(discharge)}
\end{cases}
\end{equation}
The open circuit voltage $U_{ocv} [V]$, the internal charging and discharging resistances $R_{c, int} [Ohm]$ and $R_{d,int} [Ohm]$, and the maximal charging and discharging powers $P_{c,bat,max} [kW]$ and $P_{d,bat,max}$ $[kW]$ depend on the SOC of the battery. 

The system controls are the charging and discharging powers of the battery $P_{c, bat} [kW]$ and $P_{d, bat}$ $[kW]$. 
These values are positive by definition and physically bounded, which is also true for the SOC:
\begin{align}
\label{eqn: constraints 1}
&0 \leq P_{c, bat} \leq P_{c, bat, max}(x) \\
\label{eqn: constraints 2}
&0 \leq P_{d, bat} \leq P_{d, bat, max}(x) \\
\label{eqn: constraints 3}
& x \in [0,1]
\end{align}
 
Such a model implies non-linear transfer efficiencies. In particular, the charging speed $\dot{x}$ is not a linear function of the (dis)charging power and the SOC. These realistic conditions may have an influence on the optimal strategies.

\subsection{State and action spaces}
Given the elements that appear in the cost functions \eqref{eq: cost function crit 1}, \eqref{eq: cost function crit 2}, \eqref{eq: cost function crit 3}, we consider for the state space of our RL agents the time step $\tau \in \mathcal{T}=\{0, 1, \dots, H-1\}$
(time is necessarily discrete in the MDP framework),
the state of charge $x \in \mathcal{S}o\mathcal{C} = [0, 1]$ and the highest demand peak registered so far during the current billing period $p\in \mathcal{P} = [0, p_{max}]$. 
We also add the difference between the electricity demand and the solar production $\delta=P_{cons}-P_{pv} \in \Delta = [-\delta_{min}, \delta_{max}]$, as we expect optimal decisions to depend on the current production and consumption. 
% Otherwise, the same sequence of actions would be performed for any day. 
Without, only the highest demand peak $p$ could differentiate the days.
$\delta_{min}, \delta_{max}$ and $p_{max}$ are parameters extracted from the data. 

The action space 
% or the environment 
must ensure \eqref{eqn: constraints 1}-\eqref{eqn: constraints 3}. Action $a [kW]$ is defined as $a=P_{c,bat}-P_{d,bat}$, and hence charging power $P_{c,bat} = a^{+}$ and discharging power $P_{d,bat} = a^{-}$.  As we have observed that small charging or discharging powers have higher battery efficiencies, we simplify the mixed state-control constraints \eqref{eqn: constraints 1}-\eqref{eqn: constraints 2} by a simple bound constraint $\mathcal{A}=[a_{min}, a_{max}]$ with 
\begin{align}
    a_{max} &= \underset{x \in [0, 1]}{\text{min}}\, P_{c,bat,max}(x) \\
    a_{min} &= -\underset{x \in [0, 1]}{\text{min}}\, P_{d,bat,max}(x)
\end{align}
so that the action space does not depend on the state of charge. 
% A positive value of $a\in \mathcal{A}$ corresponds to a charge, a negative one to a discharge.

Since we will apply a method derived from tabular Q-learning, we discretize the state and action spaces, and denote the discretized spaces by $\mathcal{S}o\mathcal{C}_d$, $\Delta_d$ and $\mathcal{P}_d$ and the discretized action space by $\mathcal{A}_d$.

The discrete time space coincides with the sampling times of the average electricity demand $P_{cons}$ and average electricity production $P_{pv}$ measurements. In other words, time step $\tau$ corresponds to real time $t=\tau\Delta t$. 



\subsection{Search for an optimal policy }
\label{subsection: search for an optimal policy}
To compute an optimal policy, we choose to apply a policy iteration (PI)  algorithm \cite{Policy_Iteration}. The main idea of PI algorithms is to improve an initial policy $\pi_0$ by alternating evaluation and improvement steps until no better policy can be found.

At iteration $k$, the evaluation step consists in computing $Q^{\pi_k}(\tau, s,a)$ for all time $\tau\in\mathcal{T}$ and state-action pairs $(s,a)\in \mathcal{S}\times \mathcal{A}(s)$. This is the unique fixed point of Bellman equation with policy $\pi$:
\begin{equation}
    \label{eq: Bellman equation with policy}
    Q^\pi(\tau, s,a)=\mathbb{E}_\mathcal{P}\left[ \mathcal{C}_\tau(s,a,s') + Q^\pi(\tau', s', a')\, \right]
\end{equation}
where $\tau'=\tau+1$, $Q^\pi(H, \cdot, \cdot)=0$, $s'\sim \mathcal{P}(s,a)$ and $a' \sim \pi(\tau', s')$. 
This can be done by dynamic programming in perfectly deterministic environments.
% , or similarly to \eqref{eq: Q-learning update}:
% \begin{align}
%     \label{eq: Q-function evaluation}
%     &\hat{Q}^{\pi_k}_{l+1}(\tau_l,s_l, a_l) = \hat{Q}^{\pi_k}_{l}(\tau_l,s_l,a_l) + \alpha(n_{\tau_l,s_l,a_l}) TD_l \\
%     &\forall (\tau, s, a) \neq (\tau_l, s_l, a_l), \hat{Q}^{\pi_k}_{l+1}(\tau, s, a) = \hat{Q}^{\pi_k}_{l}(\tau, s, a)
% \end{align}
% with $TD_l$ the temporal difference error defined as:
% \begin{equation}
%     \begin{aligned}
%         TD_l &= \mathcal{C}_{\tau_l}(s_l, a_l ,s_{l+1}) \\
%         &\quad + \hat{Q}^{\pi_k}_{l}(\tau_{l+1},s_{l+1},\pi_{l}(\tau_{l+1},s_{l+1})) -  \hat{Q}^{\pi_k}_{l}(\tau_l,s_l,a_l)
%     \end{aligned}
% \end{equation}

Still at iteration $k$, the policy improvement step is done by computing \begin{equation}
    \label{eq: policy improvement}
    \pi_{k+1}(\tau,s)=\underset{\tilde{a}\in \mathcal{A}(s)}{\text{argmin}}\, Q^{\pi_k}(\tau,s,\tilde{a})
\end{equation} for all time $\tau\in\mathcal{T}$ and state $s\in \mathcal{S}$.

As long as all transitions are tested and the evaluation is correct, the policy iteration algorithm converges to an optimal policy.

\medskip

To simplify the minimization problems, we will split the training into separate days. 
We define the $Q$-function for policy $\pi$ knowing the power demand and production of day $d\in\mathcal{D}$ as:
\begin{equation}
    \label{eq: Q-function for day d}
    Q_d^\pi=\mathbb{E}_{\mathcal{P}}\left[ Q^\pi | \{P_{pv}(\tau), P_{cons}(\tau)\}_{\tau\in \mathcal{T}} \right]
\end{equation}
 
% We choose to apply Policy Iteration to find the optimal policy.
Our policy improvement step is classical, given by \eqref{eq: policy improvement}. The evaluation step is adapted for the training split and is described in Alg. \ref{alg: evaluation step}

\begin{algorithm}
\caption{Evaluation step $k$}\label{alg: evaluation step}
\begin{algorithmic}
\State{$\hat{Q}^{\pi_k} \leftarrow 0$}
\For{each $d_i \in \mathcal{D}, 1 \leq i \leq   |\mathcal{D}|$}
\State{Compute $Q_{d_i}^{\pi_k}$ (through dynamic programming)}
\State{$\hat{Q}^{\pi_k} \leftarrow \hat{Q}^{\pi_k} + \frac{1}{i} \left[ Q_{d_i}^{\pi_k} - \hat{Q}^{\pi_k}\right]$}
\EndFor
\end{algorithmic}
\end{algorithm} 

Let us now clarify the computation of $Q_d^\pi$. We have access to a simulator \eqref{eqn:x_dot} that reproduces the system well enough. For any given day, we only need to feed the collected production $P_{pv}$ and consumption $P_{cons}$ data to the simulator to retrospectively sample any transition.
With the specific knowledge about day $d$, the minimization problem limited to that day becomes deterministic. We can then use DP derived from equation \eqref{eq: Bellman equation with policy} to compute the function $Q_d^\pi$. 

 Estimation $\hat{Q}^{\pi}$ from Alg. \ref{alg: evaluation step} converges to $\mathbb{E}\left[ Q^\pi_d \right]$ when the number of training days grows to infinity. Then,
\begin{equation}
\begin{aligned}
    \mathbb{E}_\mathcal{D}\left[ Q_d^{\pi}(\tau,s,a) \right]&= \mathbb{E}_\mathcal{D}\left[ \mathcal{C}_\tau(s,a,s')+ Q_d^\pi(\tau', s', a') \right] \\
    &= \mathbb{E}_{\mathcal{P}}\left[ \mathcal{C}_\tau(s,a,s') + Q^\pi (\tau', s', a') \right]
\end{aligned}
\end{equation}with $ a' \sim \pi(\tau', s')$. So, $Q^\pi=\mathbb{E}\left[ Q^\pi_d \right]$ is a fixed point of \eqref{eq: Bellman equation with policy}, which proves the correctness of the evaluation.

\subsection{Efficient choice of initial policy} 
To speed up the training, we want to find an initial policy $\pi_0$ close to $\pi^*$. 

% Indeed, when the production and the consumption of a day are known, the minimization problem that is limited to that day becomes deterministic and can be solved with classical DP based on \eqref{eq: Bellman optimality equation}. 
Let us denote the optimal Q-function associated to day d as $Q^*_d$. This function is defined as follows:
\begin{equation}
    \label{eq: optimal Q-function for day d}
    Q_d^*=\mathbb{E}_{\mathcal{P}}\left[ Q^* | \{P_{pv}(\tau), P_{cons}(\tau)\}_{\tau\in \mathcal{T}} \right]
\end{equation}
It can be computed similarly to $Q_d^\pi$ with classical DP based on \eqref{eq: Bellman optimality equation} knowing the production and consumption associated to day $d$. 

We propose to initialize the PI algorithm with an average of these optimal Q-functions $Q^*_d$. This average can be estimated iteratively as follows: 
\begin{equation}
    \bar{Q}_{n+1} = \bar{Q}_{n} + \alpha(n+1) \left[ Q^*_{d_n} - \bar{Q}_{n}\right]
\end{equation}
with $\alpha: \mathbb{N}^* \to \mathbb{R}^*_+$ a learning rate such as $n \mapsto 1/n$.

% On a side note, using that learning rate means computing the mean of all $Q^*_d$. Therefore, parallelization is possible.

$\bar{Q}_n$ converges under mild conditions on $\alpha$ to $\bar{Q}$ when the number of training days grows to infinity, with $\bar{Q}$ defined as:
\begin{equation}
    \bar{Q}=\mathbb{E}_\mathcal{D}\left[Q_d^* \right]
\end{equation}

However, the latter is not a fixed point of the Bellman equation \eqref{eq: Bellman optimality equation}, but an upper bound. Indeed,
% \begin{equation}
%     \begin{aligned}
%     \bar{Q}(s,a)&\mathbb{E}\left[ \mathbb{E}\left[ \mathcal{R}(s,a,s') + \underset{\tilde{a}}{\text{max}}\, Q_d^*(s', \tilde{a}) \Big| \{P_{pv}(\tau), P_{cons}(\tau)\}_{\tau\in \mathcal{T}}  \right]  \right] \\
%     &\geq \mathbb{E} \left[ \mathcal{R}(s,a,s')+\underset{\tilde{a}}{\text{max}}\,\bar{Q}(s',\tilde{a}) \right] 
%     \end{aligned}
% \end{equation}
\begin{equation}
    \begin{aligned}
    &\mathbb{E}_{\mathcal{D}}\left[ \mathbb{E}_\mathcal{P}\left[\underset{\tilde{a}}{\text{min}}\, Q_d^*(s', \tilde{a}) \Big| \{P_{pv}(\tau), P_{cons}(\tau)\}_{\tau\in \mathcal{T}}  \right]  \right] \\
    &\leq \mathbb{E}_\mathcal{P} \left[\underset{\tilde{a}}{\text{min}}\,\bar{Q}(s',\tilde{a}) \right] 
    \end{aligned}
\end{equation}
thus
\begin{equation}
    \bar{Q}(s,a) \leq \mathbb{E}_\mathcal{P}\left[\mathcal{C}(s,a,s')+ \underset{\tilde{a}}{\text{min}}\,\bar{Q}(s',\tilde{a}) \right] 
\end{equation}
but we can expect it to be relatively close to the optimal $Q$-function $Q^*$. Thus, we choose $\pi_0(\tau, s, a)=\underset{\tilde{a}}{\text{argmin}}\, \bar{Q}_D(\tau, s, \tilde{a})$ as initialization for the PI algorithm, where $D$ is the number of training days.



==> content/backgroundv2.tex <==
\label{section 3}

\subsection{Reinforcement learning}
In Reinforcement Learning, an agent (i.e. decision-maker) attempts to learn an optimal behavior through a trial and error process based on the costs (or rewards) received from its interactions with an environment. 
% Specifically, its goal is to find an optimal mapping from states to actions with respect to a cost (or reward) function. 

We focus on discrete-time stochastic control processes. An agent is considered to follow a finite horizon Markov Decision Process (MDP), which is defined by the following five elements:
\begin{itemize}
\item a finite horizon $H \in\mathbb{N}$: the time $\tau$ belongs to $\mathcal{T}=\{0, 1, \dots, H-1\}$.
    \item a state space $\mathcal{S}$ encompassing the possible states of the agent. It represents the elements on which the agent bases its action. For clarity's sake, we will show the time $\tau$ even though $\tau$ could be part of $s$.
    \item an action space $\mathcal{A}$ representing the actions available to the agent. $\mathcal{A}(s)$ denotes the allowed actions in state $s$ and does not depend on the time $\tau$.
    \item 
    % a distribution $\mathcal{P}$ on the next state $s'$ knowing the present state $s$ and chosen action $a$: $s'\sim \mathcal{P}(s,a)$ considered here time-invariant.
    a distribution $\mathcal{P}$ on the transitions: next state $s'$ at time $\tau + 1$ follows $\mathcal{P}(s,a)$  when performing action $a$ in state $s$ at time $\tau$.
    \item a cost function $\mathcal{C}:\mathcal{T}\times\mathcal{S}\times\mathcal{A}\times\mathcal{S}\to \mathbb{R}$ such that $\mathcal{C}_\tau(s, a, s')$ is the cost received for the transition from state $s$ to state $s'$ through action $a$ at time $\tau$. 
\end{itemize}

% The actions chosen by an agent are dictated by its policy, which is in all generality a function 
% $\pi$ mapping the time and state spaces $\mathcal{T}\times\mathcal{S}$ with the set of probability distributions on the actions $\mathcal{A}$. 
The action $a$ chosen by an agent is dictated by its policy: in state $s$ at time $\tau$, $a \sim \pi(\tau,s)$, $a\in \mathcal{A}(s)$. When the policy is deterministic, $\pi(\tau,s)$ is a Dirac delta function: $\pi(a |\tau, s)=1$. 
% In this case, we prefer  to write $\pi:\tau,s\in\mathcal{T}\times\mathcal{S}\mapsto a\in \mathcal{A}(s)$, so that 
% $\pi(\tau,s)=a$.
In this article, we work with deterministic policies.

The agent tries to find a policy $\pi^*$ minimizing the expectation 
% of its total cost over a time horizon  $H$
of its return:
\begin{equation}
    \label{eq: expected return}
    \forall \tau\in\mathcal{T}, \quad \pi^*=\underset{\pi}{\text{argmin}}\; \mathbb{E}\left[ \sum_{k=\tau}^{H-1} \mathcal{C}_k(s_k, a_k, s_{k+1}) \right] 
\end{equation}
where $(s_0, a_0, s_1, a_1, \dots, s_H)$ is an agent's trajectory following policy $\pi$: $a_k \sim \pi(k, s_k)$ and $s_{k+1} \sim \mathcal{P}(s_k, a_k)$. 

RL algorithms can be model-free or model-based. In the first case, the transition distribution $\mathcal{P}$ is not known. An agent learns to optimize its policy without intermediate modeling of the environment. In the second case, the transition distribution is known, or learned, and used as the environment model.

\subsection{$Q$-learning}
Based on the expression of the expected return \eqref{eq: expected return}, we can define for policy $\pi$ a $Q$-function such that for all $\tau, s, a \in \mathcal{T}\times\mathcal{S}\times\mathcal{A}(s)$,
\begin{equation}
\hspace*{-0.31cm} 
    Q^\pi(\tau,s,a)=\mathbb{E}\left[ \sum_{k=\tau}^{H-1} \mathcal{C}_k(s_k, a_k, s_{k+1}) \Big| s_\tau = s, a_\tau=a\right]
\end{equation}
mapping for each time $\tau$ and state-action couple $(s,a)$ the expected value of choosing action $a$ in state $s$ starting at time $\tau$ and following policy $\pi$ afterwards: for $k\in\mathcal{T}, k>\tau$, $a_k \sim \pi(k,s_k)$.

The optimal $Q$-function $Q^*$ is defined as:
\begin{equation}
    \label{eq: Q^*}
    \forall (\tau,s,a) \in \mathcal{T}\times\mathcal{S}\times \mathcal{A}(s), Q^*(\tau,s,a) = \underset{\pi}{\text{min}}\, Q^\pi(\tau,s,a)
\end{equation}
It is a fixed point of Bellman optimality equation:
\begin{equation}
    \label{eq: Bellman optimality equation}
    Q^*(\tau, s,a)=\mathbb{E}\left[ \mathcal{C}_\tau(s,a,s') + \underset{\tilde{a}\in \mathcal{A}(s)}{\text{min}} Q^*(\tau', s', \tilde{a})\, \right]
\end{equation}

Knowing $Q^*$, an optimal policy $\pi^*$ can be derived by selecting for any state $s$ and time $t$ the action $a^*\sim\pi^*(\tau, s)=\underset{a\in\mathcal{A}(s)}{\text{argmin}}\, Q^*(\tau, s, a)$.

 Watkin and Dayan's $Q$-learning algorithm returns an estimator $\hat{Q}$ of $Q^*$ that converges with probability one under mild assumptions on the exploration \cite{Q_learning}. $\hat{Q}$ stores an estimation for each state-action couple $(s, a)$. At iteration $l+1$, it is updated as follows:
\begin{align}
    \label{eq: Q-learning update}
    &\hat{Q}_{l+1}(\tau_l, s_l, a_l) = \hat{Q}_{l}(\tau_l, s_l,a_l) + \alpha(n_{\tau_l, s_l,a_l}) BE_l  \\
    &\forall (\tau, s, a) \neq (\tau_l, s_l, a_l), \hat{Q}_{l+1}(\tau, s, a) = \hat{Q}_{l}(\tau, s, a)
\end{align}
with $BE_l$ the Bellman error defined as:
\begin{equation}
    \begin{aligned}
        BE_l &= \mathcal{C}_{\tau_l}(s_l, a_l ,s_{l+1}) \\
        &\quad + \underset{\tilde{a} \in \mathcal{A}(s_{l+1})}{\text{min}}\,\hat{Q}_{l}(\tau_{l+1}, s_{l+1},\tilde{a}) -  \hat{Q}_{l}(\tau_l,s_l,a_l)
    \end{aligned}
\end{equation}
and where $\left\{ (\tau_l, s_l, a_l, s_{l+1})\right\}_{l}$ are sampled transitions using an exploration policy $\pi_{exp}$, $\alpha(l)$ is a non-increasing learning rate (typically, $\alpha(l) = 1/l$)  and $n_{\tau,s, a}$ counts the number of times the estimation of the state action pair $(\tau,s,a)$ has been updated.


$Q$-learning is off-policy: the exploration policy $\pi_{exp}$ used by the agent to explore the environment and the policy $\pi_k$ defined by $\forall (\tau,s) \in \mathcal{T}\times\mathcal{S}, \pi_k(\tau,s)=\underset{a\in \mathcal{A}}{\text{argmin}}\; \hat{Q}_k(\tau, s, a)$ are decoupled. As long as the exploration policy $\pi_{exp}$ tests all state-action pairs sufficiently, convergence is assured.

==> content/conclusion.tex <==
\label{section 6}
%\subsection{Conclusion}
We introduced a new reinforcement learning algorithm for energy and demand charges minimization. As no hyperparameters are involved and no production or consumption forecasts are required, this method is particularly simple to implement.
We showed that significant benefits can be achieved 
through intelligent battery steering, especially when demand charges are involved. 
We compared daily demand charges to monthly one and showed that the former can lead to lower power demand peaks and offers bigger potential economic gains. 
% Thus, daily demand charges yield more benefits for both utilities and end-users.

%\subsection{Future works}
The recoupling of days remains a difficult open question that has been highlighted by the consideration of battery non-linearities. Future work could focus on this aspect, as well as on the implementation of RL methods for continuous state and action spaces.


==> content/experiments.tex <==
\label{section 5}
We test our approach with a building of IFPEN's Solaize site equipped with a solar panel and a battery.
 
\subsection{Problem decomposition}
\label{problem decomposition}
As mentioned in \ref{subsection: search for an optimal policy}, the training is split into separate days. The agents are trained on a finite horizon $H$ corresponding to one day starting at midnight.
With such a split, it is optimal for an agent to have an empty battery at the end of the day. If the battery was not empty, the remaining energy could have met the electricity demand or been sold. Therefore, we choose to set the state of charge to zero at the beginning of the day.

This decomposition can result in suboptimal actions. If the battery sells electricity at the end of one day and buys it back at the beginning of the next, and the selling prices are lower than the purchase prices, it would have been more economical to store that energy. We will discuss the issue of recoupling later in section \ref{recoupling subsection}.

\subsection{Numerical settings}
We have access to two years data of PV production and power demand, with a sample time of 10 minutes.
Since the power demands vastly differ between working and non-working days, we consider them separately. In this paper, we present results on working days, where a much greater bill reduction is possible compared to non-working days. For monthly demand charges, we consider billing periods of four weeks, i.e. $20$ working days.  

The agents are trained offline over $N_{train}=300$ working days with learning rate $\alpha(n)=1/n$ and tested over $N_{test}=100$ working days. 

We will use $\mathcal{T}=\{0, 1, \dots, 143\}$, i.e. one time step every ten minutes, as it is the time interval between two successive measurements, $\mathcal{S}o\mathcal{C}_d = \{0, 0.01, \dots, 1\}$, $\Delta_d = \{-60, -58, \dots, 60\}$, $\mathcal{P}_d = \{0, 1, \dots, 100\}$ and $\mathcal{A}_d=\{-20, -19, \dots, 20\}$. 
For the simulation model \eqref{eqn:x_dot}, experimental data of $U_{ocv}$, $R_{c,int}$, $R_{d,int}$, $P_{c,bat,max}$ and $P_{d,bat,max}$ are used. $Q_{bat}^{nominal}$ is calculated from these measurements.
% $Q_{bat}^{nominal}$, $U_{ocv}$, $R_{c,int}$, $R_{d,int}$, $P_{c,bat,max}$ and $P_{d,bat,max}$ were computed using Guzzella et al's work \cite{Dynamic of the battery} on \textcolor{red}{battery: model?}.

% To compare the pricing strategies \eqref{eq: cost function crit 2} and \eqref{eq: cost function crit 3} in a meaningful way, we set $\mu_m = 20 \mu_d$, since we focus on the working days of four weeks to represent monthly demand charge assessments.

% For energy charges, the selling price is $0.098/kWh$ at all times and the selling price is equal to $0.1330/kWh$ during off-peak hours and $0.1936/kWh$ during peak hours (6:00 a.m. to 9:00 a.m. and 6:00 to 9:00 p.m.). For demand charges, the price is $\mu_d=0.5\$/kW$ for daily assessments and $\mu_m=10\$/kW$ for monthly evaluations.

Energy and demand charge prices appear in Tables \ref{table: energy charges} and \ref{table: demand charges}. On-peak hours are from 6am to 9am and 6pm to 9pm.

\medskip

\begin{minipage}[c]{\columnwidth}
\centering
\begin{tabular}{ |c|c|c| } 
 \hline
 selling price & on-peak price & off-peak price \\ 
 \hline 
 $0.098 \$/kWh$ & $0.1936 \$/kWh$ & $0.1330 \$/kWh$ \\ 
 \hline
\end{tabular}
\captionof{table}{Prices for energy charges}
\label{table: energy charges}
\end{minipage}

\begin{minipage}[c]{\columnwidth}
\centering
\begin{tabular}{ |c|c| } 
 \hline
 daily demand charges & monthly demand charges \\ 
 \hline
 $\mu_d=0.5 \$/kW$ & $\mu_m=20\mu_d=10 \$/kW$\\ 
 \hline
\end{tabular}
\captionof{table}{Prices for demand charges}
\label{table: demand charges}
\end{minipage}

\medskip

 The battery used for our numerical experiment has a storage capacity of $27.3$ kWh, costing roughly $\$4000$ given the current price per kWh.

 We introduce an heuristic controller, which will be combined to RL agents to control the system when dealing with states that were never visited during the training. The heuristic is defined as follows: the battery is charged when production is higher than consumption. When it is full, the excess power is sold. The battery is discharged when consumption is higher than production, but only during on-peak hours. At the end of the day, the battery is emptied. 



In the following, the bill reduction is defined as the difference between the bill in the no-battery case and the minimized bill.

\subsection{Comparison of agents having different state-spaces: energy charges minimization}
In this section, we treat the energy minimization problem \eqref{eqn: demand charge min} to determine the best state space for future experiments. We will use agents based on different state spaces and select the one yielding the best results.
 


% Agents $A_1$, $A_2$ and $A_3$ will have as state spaces $S_1=\mathcal{T} \times \mathcal{S}o\mathcal{C}_d$, $S_2=\mathcal{T} \times \mathcal{S}o\mathcal{C}_d \times \{-1, 0, 1\}$ and $S_3=\mathcal{T} \times \mathcal{S}o\mathcal{C}_d \times \Delta_d$ respectively and will be trained with cost function \eqref{eq: cost function crit 1}. 
Three agents with different state spaces are trained with cost function \eqref{eq: cost function crit 1}. Agent $A_1$ has state space $S_1=\mathcal{T} \times \mathcal{S}o\mathcal{C}_d$, agent $A_2$ has state space $S_2=\mathcal{T} \times \mathcal{S}o\mathcal{C}_d \times \{-1, 0, 1\}$ and agent $A_3$ has state space $S_3=\mathcal{T} \times \mathcal{S}o\mathcal{C}_d \times \Delta_d$.
The last element of $S_2$ indicates whether there is an excess of consumption or of production. During the tests, when a state has never been visited during the training, the agents do nothing: there is no charge nor discharge.

% We also consider 
% % a simple heuristic against which our results will be compared. This heuristic works as follows:
% the following simple heuristic: the battery is charged when production is higher than consumption. When it is full, the excess power is sold. The battery is discharged when consumption is higher than production, but only during on-peak hours. At the end of the day, the battery is emptied. 

We further introduce agent $A_4$ that is identical to $A_3$, except that it follows the heuristic during the test phase for states that were never visited during the training phase. 

In Fig. \ref{fig:bill minimization}, we show for each day of our test set the bill reduction obtained with the heuristic and agents $A_1$-$A_4$.  
We observe that the average profits increase non-trivially with the complexity of the state spaces. 
Since state space $S_3$ gives the best results, we will use it as a basis for all other experiments. 

Comparing agent $A_3$ and agent $A_4$, the addition of the heuristic brings negligible additional benefits. It indicates that few states have not been visited during the training.

\begin{figure}
    \centering
    \includesvg[width=0.8\columnwidth]{img/cons_min.svg}
    \caption{Swarm plot representing the daily bill reductions on the test set when using our agents versus no battery. 
    % A swarm plot is a categorical scatter plot with adjusted points so that they do not overlap. The horizontal distribution within a class does not have any particular meaning. 
    Each color represents one month.}
	\label{fig:bill minimization}
\end{figure}


\subsection{Daily demand charge minimization}
\label{subsection: daily DC}
Agent $A_5$ lives in $S_5=\mathcal{T} \times \mathcal{S}o\mathcal{C}_d \times \Delta_d \times \mathcal{P}_d$ and is trained with cost function \eqref{eq: cost function crit 2}. Agent $A_6$ is based on the same policy, except that it follows the mentioned heuristic for states that were not visited during the training.

We show in Fig. \ref{fig: daily based bill improvement} the bill reductions of the heuristic, agent $A_5$ and agent $A_6$. We note that our RL agents are systematically beneficial.
% The magnitude of the gains is much larger than in the previous experiment with energy loads only: the maximum gain is much higher, the minimum gain is lower. 
Only the heuristic failed at least once to reduce the bill. The difference between the use or not of the heuristic remains very small. The average daily gains amount to $\$3.26$ for agent $A_5$ and $\$3.34$ for agent $A_6$.  

\begin{figure}
    \centering
    \includesvg[width=0.8\columnwidth]{img/daily_dc_improvement.svg}
    \caption{Swarm plot representing the bill reductions on the test set for the heuristic, agents $A_5$ and agent $A_6$.}
	\label{fig: daily based bill improvement}
\end{figure}

We highlight typical days with good and weak bill reduction in Fig. \ref{fig: good and bay day for daily DC}. 
For the day with a big bill reduction, $\$2.64$ are spared on energy charges and $\$5.0$ are spared on demand charges, for a total bill reduction of $\$7.64$. In such a day, the sudden production fall during high consumption period can introduce high peak demand. The battery charged during low consumption period (at the beginning of the day) then allows to significantly reduce the demand charges.
For the day with a small reduction, $\$1.99$ are saved on energy charges while $\$1.0$ are lost on demand charges, for a total bill reduction of $\$0.99$. In these kind of days, the battery is charged before the first on-peak hours to absorb the on-peak consumption and to deal with potential important peak demands. This strategy appears natural since the peak demand during high consumption period risks to increase significantly the electricity bill (like in the big bill reduction case). Unfortunately, this decision increases slightly the demand charge when the high loads are totally covered by solar production.

 An interesting observation is that the battery has not had enough time to fully charge before the first on-peak hour. The speed of charge is likely limited to keep small demand charges. This indicates that the benefits of having a bigger battery for the first on-peak hours may be limited. They are more clear for the second on-peak hours when we look at \ref{fig: good day daily DC}, as the power demand is not always close to zero.
 % The choice of starting the day at midnight imposes an empty battery at that time. A beginning at the end of the last on-peak hours may leave more time to the battery to charge.
 In addition, this observation suggests that the problem decomposition described in \ref{problem decomposition} may not be optimal. We are to discuss in section \ref{recoupling subsection} the potential improvements on this issue.
 
 
 % Energy charges are weaker on the typical bad days mainly because it is much sunnier: the battery is much less depleted during the second on-peak hours. There is smaller need to shift power demand from on-peak to off-peak hours than for the other day. 

 % Demand charges increase for the bad day, as the battery is initially loaded to spare energy charges later on and there is no demand peak to flatten. The good day comes with huge demand charges reduction, because of a big surge in power demand between time steps $90$ and $100$: the battery efficiently limits the call to the grid.



 

\begin{figure}
    \centering
     \hspace*{-0.3cm}
     \begin{subfigure}[b]{0.5\columnwidth}
         \centering
         \includesvg[width=\textwidth]{img/bad_day_daily_DC.svg}
         \caption{Day with small bill reduction}
         \label{fig: bad day daily DC}
     \end{subfigure}
     \begin{subfigure}[b]{0.5\columnwidth}
         \centering
         \includesvg[width=\textwidth]{img/good_day_daily_DC.svg}
         \caption{Day with good bill reduction}
         \label{fig: good day daily DC}
    \end{subfigure}
    \caption{Typical days with small and good bill reduction. Top figures show the power generation, the electricity demand and the state of charge of the battery. Bottom figures represent $P_{meter}$ with and without battery. Gray areas correspond to on-peak hours.}
    \label{fig: good and bay day for daily DC}
\end{figure}


\subsection{Monthly demand charge minimization}
\label{subsection: monthly DC}
Similar to the previous section, agent $A_7$ lives in $S_5=\mathcal{T} \times \mathcal{S}o\mathcal{C}_d \times \Delta_d \times \mathcal{P}_d$ with cost function \eqref{eq: cost function crit 3}. Agent $A_8$ follows the same policy, except during the test phase for non-visited states, in which it follows the heuristic.

The demand charges are computed for the whole billing period (i.e. the working days of four weeks). To obtain daily bills that can be plotted like in Fig. \ref{fig: daily based bill improvement}, we divide the monthly demand charge by the number of working days ($20$) and add it to the energy charge.

Our results are shown in Fig. \ref{fig: month-based bill minimization}. Maximum gains are again much higher than with energy charges minimization. Once more, we observe that our agents are systematically beneficial, and the difference between the use or not of the heuristic remains marginal.
% but that time the difference between the use or not of the heuristic is smaller: the average daily gains amount to $\$3.09$ for agent $A_7$ and $\$3.10$ for agent $A_8$. Also, the heuristic never loses money.


\begin{figure}
    \centering
    \includesvg[width=0.8\columnwidth]{img/monthly_dc_improvement.svg}
    \caption{Swarm plot representing the daily bill reductions on the test set for the heuristic, agent $A_7$ and agent $A_8$.}
	\label{fig: month-based bill minimization}
\end{figure}

We show in Fig. \ref{fig: good and bay day for monthly DC} typical days with small and big bill reductions. For the day with a small reduction, $\$0.71$ are spared on energy charges while $\$0.5$ are lost on demand charges, for a total bill reduction of $\$0.21$. For the day with a big bill reduction, $\$3.04$ are spared on energy charges and $\$5.0$ are spared on demand charges, for a total bill reduction of $\$8.04$. 

The day with a small bill reduction (Fig. \ref{fig: bad day monthly DC}) is the first of its billing period. We can observe that the agent's behavior is cautious: the power demand never exceeds $20 kW$. The loose on demand charges can be caused by another day of the billing period. 

For the day with good bill reduction (Fig. \ref{fig: good day monthly DC})a higher peak of $20 kW$ has been measured earlier in the billing period. We can see that 
% the agent is not that cautious with demand charges:
the power demand is instantly bigger and allows the battery to be fully charged before the first on-peak hours, leading to smaller power demands during the first on-peak hours. 
% A higher peak of $20 kW$ has been measured earlier in the billing period. 

 These results correspond to the intuition. Before a high peak is reached during the billing period, the conservative behavior limits the economies with energy charges. Afterwards, electricity demands are less restrictive and the peak load to the grid is less reduced. 

 % Days like the one on Fig. \ref{fig: good day monthly DC} require a bigger battery as the demand power is not null during the on-peak hours. Days like the one on the left, probably with a bad weather, do not.


\begin{figure}
    \centering
    
     \hspace*{-0.3cm}
     \begin{subfigure}[b]{0.5\columnwidth}
         \centering
         \includesvg[width=\textwidth]{img/bad_day_monthly_DC.svg}
         \caption{Day with small bill reduction}
         \label{fig: bad day monthly DC}
     \end{subfigure}
     \begin{subfigure}[b]{0.5\columnwidth}
         \centering
         \includesvg[width=\textwidth]{img/good_day_monthly_DC.svg}
         \caption{Day with good bill reduction}
         \label{fig: good day monthly DC}
    \end{subfigure}
    \caption{Typical days with small and good bill reduction. Top figures show the power generation, the electricity demand and the state of charge of the battery. Bottom figures represent $P_{meter}$ with and without battery. Gray areas correspond to on-peak hours.}
    \label{fig: good and bay day for monthly DC}
\end{figure}


\subsection{Comparison of daily and monthly demand charges}

The average daily bill reduction is slightly bigger with daily demand charges: 
$\$3.26$ for $A_5$ and $\$3.34$ for and $A_6$ versus $\$3.09$ for $A_7$ and $\$3.10$ for $A_8$.

A quite crucial observation is that for the monthly demand charge case, month $0$ is monopolizing the very high bill reductions, whereas the highest reductions are much smaller for all the other months. The total demand charge reduction amounts to $\$100$ for month $0$, whereas it is equal to $\$0$ for month $1$ and month $2$ and $-\$10$ for month $3$ and month $4$. Without month $0$, the average economic gains would decrease considerably. Daily demand charge appears therefore more reliable for bill reduction. 


We show the distribution of the measured power demands $P_{meter}$ to the grid in Fig. \ref{fig: billing period comparison}. The blue stairs represent agent $A_6$ (daily demand charges). The red one represent agent $A_8$ (monthly demand charges).

We can note that for monthly demand charges, the numbers of high energy demand peaks increase. This suggests that daily demand charges are more likely to decrease the load on the grid.

A simple explanation is that for a given peak, the agent is not penalized as long as he does not exceed it. As explained in section \ref{subsection: monthly DC}, once a high peak has been reached with monthly demand charges, the consumer can be less motivated to reduce its peak demand for the rest of the month, and thus leads to more demand peaks. 
% Therefore, the agent is free to rely on high energy demands to minimize the energy consumption. The longer the billing period is, the more free the agent is. 

\begin{figure}
    \centering
    \includesvg[width=0.8\columnwidth]{img/DC_comparison.svg}
    \caption{Histograms of the power provided by the grid (kW) measured on intervals of 10 minutes for demand charges evaluated on a monthly and on a daily basis.}
	\label{fig: billing period comparison}
\end{figure}

\subsection{Re-coupling}
\label{recoupling subsection}
We have trained our agents by decoupling the days as described in section \ref{recoupling subsection}. In section \ref{subsection: daily DC}, we have mentioned that there may be room to increase the gains by re-coupling separate days. A first attempt at re-coupling is to charge the battery at the end of the day during the last off-peak hours. While being careful not to exceed the peak demand reached during the day, we thus extend the time the battery has to charge before the next on-peak hours.

By applying this heuristic on our trained agents, we observe an additional bill reduction for daily demand charges, but a performance degradation for monthly ones. We achieve a mean daily bill reduction of $\$3.65$ for daily demand charges ($\$3.10$ for monthly demand charges), meaning the battery pays for itself in 3 years. One explanation is the use of higher charging powers for the latter. In our non-linear battery model, the charging speed $\dot{x}$ grows sub-linearly with the charging power $P_{c,bat}$. Conversely, $\dot{x}$ decreases super-linearly when the discharging power $P_{d,bat}$ increases. The faster the charges and discharges, the more power losses they cause.



 

==> content/introductionv2.tex <==
In the European spot electricity market, the price is determined by the marginal cost of the most expensive power plant in operation \cite{Basics_Electricity_Price_Formation}. Thus, high peak demand often requires the use of more expensive and much more polluting power generators, such as coal and natural gas \cite{Relation_price_pollution}. It is therefore in the interests of energy suppliers and society to reduce the peak demand so that the most expensive generators are used as little as possible. 

Mechanisms to motivate customers to change their consumption behaviors are referred to as demand-side management \cite{Demand_Side_Management}. A common one for smoothing demand curves is the implementation of time-of-use (TOU) pricing \cite{Time_of_Use_pricing} with on-peak and off-peak hours. US utilities have further introduced demand charges to encourage large-load customers (usually commercial or industrial ones) to flatten their load curves \cite{Demand_Charges}. The electricity bill consists of three parts: a fixed subscription fee, an energy charge depending on the TOU pricing, and a demand charge according to the maximal power demand during the billing period. The billing period can be one month or one day \cite{daily_monthly_DC}.
While monthly demand charges may allow utilities to definitely shut down certain high-cost power plants, the daily demand charge was designed to reduce customers’ exposure to high demand charges.
% Intuitively, once a high peak has been reached with monthly demand charges, the consumer can be less motivated to smooth its power demand for the rest of the month. 
 
To reduce the peak demand, numerous technologies have been developed \cite{SOTA_of_Peak_Shaving_Review}. A common one is the use of energy storage devices, such as a battery.

In this article, we focus on minimizing the electricity bill. The consumer has a Lion battery and self-owned solar power generation. The main difficulties come from the uncertainties of future electricity generation and consumption and that the peak demand is observed only after the whole billing period.




Classic methods, such as linear-quadratic regulators \cite{Temperature_forecasts} and model predictive control \cite{Radiation_forecasts, Augmented_state_space}, require forecasts of electricity production and consumption. Their performances rely on the quality of previsions. Though, it is difficult to built precise forecasting models for renewable power generation \cite{Energy_forecasts} and individual electricity demand \cite{Demand_forecasts}. 
Alternatively, an online control based on Lyapunov optimization for commercial buildings was introduced \cite{Lyapunov_Optimization}. That solution does not require production and consumption forecasts. However, an upper bound to the electricity bill is minimized: the objective function is a weighted sum of the bill and a Lyapunov drift. That sum is controlled by a hyperparameter that must be tuned.


Reinforcement learning (RL) methods provide a model-free alternative. By trial and error, they learn optimal battery control strategies from
observations of the system’s output.
RL has been successfully applied to the problem of energy charges minimization in various settings (see e.g. \cite{EC1, EC2, EC3}). However, accounting for demand charges is challenging: they constitute a sparse signal that depends on the entire billing period history.



To address this issue, we propose a reinforcement learning algorithm with a designed cost function that only depends on the current state and action, similarly to \cite{Augmented_state_space}. The algorithm estimates future expected costs in a tabular setting and use them to determine optimal actions. Though the convergence to optimal controllers is guaranteed in the tabular setting, the convergence is known to be very slow. 
We propose an off-line training using dynamic programming (DP) on deterministic transitions that accelerates the convergence, is simple to implement and does not need fine hyperparameter tunings. 

We note that once trained off-line with collected production and consumption data, the RL controllers can be used online to reduce electricity bills. Moreover, the trained controllers can be progressively improved with new collected data. This allows them to automatically adapt to either new consumption patterns of the customer or production changes caused by climate changes.

The remainder of this paper is organized as follows. Section \ref{section 3} provides background on reinforcement learning. Section \ref{section 4} formalizes electricity bill minimization problems and presents how we apply reinforcement learning. Section \ref{section 5} shows economical benefits of our method in several contexts. Section \ref{section 6} summarizes our results and discusses possible improvements.


